HuViDPO:Enhancing Video Generation through Direct Preference Optimization for Human-Centric Alignment

With the rapid development of AIGC technology, significant progress has been made in diffusion model-based technologies for text-to-image (T2I) and text-to-video (T2V). In recent years, a few studies have introduced the strategy of Direct Preference Optimization (DPO) into T2I tasks, significantly enhancing human preferences in generated images. However, existing T2V generation methods lack a well-formed pipeline with exact loss function to guide the alignment of generated videos with human preferences using DPO strategies. Additionally, challenges such as the scarcity of paired video preference data hinder effective model training. At the same time, the lack of training datasets poses a risk of insufficient flexibility and poor video generation quality in the generated videos. Based on those problems, our work proposes three targeted solutions in sequence. 1) Our work is the first to introduce the DPO strategy into the T2V tasks. By deriving a carefully structured loss function, we utilize human feedback to align video generation with human preferences. We refer to this new method as HuViDPO. 2) Our work constructs small-scale human preference datasets for each action category and fine-tune this model, improving the aesthetic quality of the generated videos while reducing training costs. 3) We adopt a First-Frame-Conditioned strategy, leveraging the rich in formation from the first frame to guide the generation of subsequent frames, enhancing flexibility in video generation. At the same time, we employ a SparseCausal Attention mechanism to enhance the quality of the generated videos.More details and examples can be accessed on our website: https://tankowa.github.io/HuViDPO. github.io/.

==> sec/3_Preliminaries.tex <==
\section{Preliminaries}

\subsection{Preliminaries of Stable Diffusion}

Diffusion model generates data by reversing a gradual noising process. In the forward diffusion process, we start with real data $x_0$ and progressively add Gaussian noise at each timestep $t$ according to a predefined variance schedule. The process is defined as:

\begin{equation}
q(x_t \mid x_{t-1}) = \mathcal{N}\left( x_t; \sqrt{1 - \beta_t} x_{t-1}, \beta_t I \right).
\end{equation}

The objective of the diffusion model is to learn the reverse of the forward process, effectively denoising the data step by step. To achieve this, a neural network $\boldsymbol{\epsilon}_\theta(x_t, t)$ is trained to predict the noise $\boldsymbol{\epsilon}$ added at each timestep $t$. The simplified training loss function is given by:

\begin{equation}
\mathcal{L}_{\text{simple}} = \mathbb{E}_{t, x_0, \boldsymbol{\epsilon}} \left[ \left\| \boldsymbol{\epsilon} - \boldsymbol{\epsilon}_\theta\left( x_t, t \right) \right\|^2 \right].
\label{lab:1}
\end{equation}

where $x_t$ is computed using:

\subsection{Direct Preference Optimization}

In DPO, the objective is to derive an optimal reward function by maximizing the log-likelihood of preference pairs, thereby optimizing the policy to better match human preferences. Given a sample pair $(x, y_w, y_l)$, where $y_w$ represents the preferred sample and $y_l$ represents the less preferred sample, the probability of preference can be expressed as:

\begin{equation}
p(y_w \succ y_l \mid x) = \sigma(r^*(x, y_w) - r^*(x, y_l)).
\end{equation}

To align the generated samples with human preferences, we maximize the log-likelihood of the preference pairs. The corresponding loss function is defined as:

\begin{equation}
\mathcal{L}= -\mathbb{E}_{(x, y_w, y_l) \sim D} \left[ \ln \sigma(r^*(x, y_w) - r^*(x, y_l)) \right].
\end{equation}

In the reverse derivation of the reward function, we assume that the optimal reward function takes the form of the log-ratio between the reference policy $\pi_{\text{ref}}$ and the current policy $\pi$:

\begin{equation}
r^*(x, y) = \beta \log \frac{\pi(y \mid x)}{\pi_{\text{ref}}(y \mid x)}.
\end{equation}

By substituting this into the loss function, we obtain the final DPO loss function:

\begin{equation}
\begin{aligned}
\mathcal{L} = -\mathbb{E}_{(x, y_w, y_l) \sim D} \Big[ &\ln \sigma\Big( \beta \log \frac{\pi(y_w \mid x)}{\pi_{\text{ref}}(y_w \mid x)} \\
&- \beta \log \frac{\pi(y_l \mid x)}{\pi_{\text{ref}}(y_l \mid x)} \Big) \Big].
\end{aligned}
\end{equation}

This loss function optimizes the difference in rewards between preference pairs, allowing the model to learn behaviors that better align with human preferences.



